Learning Off-policy with Model-based Intrinsic Motivation For Active Online Exploration

Recent advancements in deep reinforcement learning (RL) have demonstrated notable progress in sample efficiency, spanning both model-based and model-free paradigms. Despite the identification and mitigation of specific bottlenecks in prior works, the agent's exploration ability remains under-emphasized in the realm of sample-efficient RL. This paper investigates how to achieve sample-efficient exploration in continuous control tasks. We introduce an RL algorithm that incorporates a predictive model and off-policy learning elements, where an online planner enhanced by a novelty-aware terminal value function is employed for sample collection. Leveraging the forward predictive error within a latent state space, we derive an intrinsic reward without incurring parameters overhead. This reward establishes a solid connection to model uncertainty, allowing the agent to effectively overcome the asymptotic performance gap. Through extensive experiments, our method shows competitive or even superior performance compared to prior works, especially the sparse reward cases.

==> sections/related_works.tex <==
\section{Related Work}
\label{sec:related_work}
%% from the perspective of model utilization and policy derivation.
\textbf{Model-based RL} is often considered more sample-efficient than its model-free counterparts~\citep{moerland2023model}. Key strategies to enhance sample complexity involve improving the UTD ratio with model-generated transitions~\citep{sutton1990integrated, mbpo/19}, building a more accurate value estimator using model rollouts~\citep{mve/18}, and computing the analytic policy gradients by back-propagating through differentiable model~\citep{svg/15, Dreamer_v1/20}. Beyond direct policy derivation, optimal policies can be obtained by planning using the dynamics model~\citep{pets/18, planet/19}. Furthermore, the methods above are not mutually exclusive but can, in principle, be complementary. For example, Dreamer~\citep{Dreamer_v1/20} derives an optimal policy using the analytic policy gradient that is back-propagating through the imagined trajectories. Approaches like \citet{polo/19, loop/21, TDMPC/22} integrate planning with the learning of a terminal value function. While combining online planning with a global policy or value function is a practical method for better policies beyond local solutions, our work explores whether an off-policy agent, enhanced with intrinsic rewards, aids planning-based policy search.

\textbf{Exploration and intrinsic motivation in RL} \ \ 
The exploration ability is crucial for a deep RL agent's performance and sample efficiency~\citep{sac/18}. A well-shaped external reward helps to guide the learning process, thus avoiding some local minima cases~\cite{DPG-R/17}. However, things become intractable when the external reward is sparse or non-existent. Inspired by intrinsic motivation in psychology~\citep{intrinsic_rl/04}, the intrinsic reward signals are proposed, which are associated with curiosity~\citep{curiosity_rl/19}, information gain~\citep{vime/16, avtive_mani/22}, uncertainty quantification~\citep{rnd/19, evd/19}, and some other novelty measurements.

Although this exploration bonus can be accessed without approximated dynamics models, proper usage of the learned model aids the identification of a wide variety of intrinsic motivation signals~\citep{corr/abs-2301-10067}. For example, ICM~\citep{icm/17} assigns an intrinsic reward based on forward dynamics prediction error, while Max~\citep{max/19} employs a model-based active exploration scheme that seeks novelty derived from the disagreements predicted by the ensemble members. Max achieves significantly more efficient exploration over high-dimensional state space than the reactive exploration methods. Our work is inspired by this active exploration framework. Still, ACE conducts online planning with a curiosity-augmented terminal value function to determine action sequences that balance exploration and exploitation trade-offs.
